Alignment of a circumbinary disc around an eccentric binary with application to KH 15D

We analyse the evolution of a mildly inclined circumbinary disc that orbits an eccentric orbit binary by means of smoother particle hydrodynamic (SPH) simulations and linear theory. We show that the alignment process of an initially misaligned circumbinary disc around an eccentric orbit binary is significantly different than around a circular orbit binary and involves tilt oscillations. The more eccentric the binary, the larger the tilt oscillations and the longer it takes to damp these oscillations. A circumbinary disc that is only mildly inclined may increase its inclination by a factor of a few before it moves towards alignment. The results of the SPH simulations agree well with those of linear theory. We investigate the properties of the circumbinary disc/ring around KH 15D. We determine disc properties based on the observational constraints imposed by the changing binary brightness. We find that the inclination is currently at a local minimum and will increase substantially before setting to coplanarity. In addition, the nodal precession is currently near its most rapid rate. The recent observations that show a reappearance of Star B impose constraints on the thickness of the layer of obscuring material. Our results suggest that disc solids have undergone substantial inward drift and settling towards to disc midplane. For disc masses $\sim 0.001 M_\odot$, our model indicates that the level of disc turbulence is low $\alpha \ll 0.001$. Another possibility is that the disc/ring contains little gas.

==> RESPONSE.tex <==
RESPONSE: We thank Hossam Aly for helpful comments that lead to the improvement of this manuscript. We have addressed all of the minor revisions and have outlined our responses below. We hope that this manuscript is now ready for publication.


Reviewer's Comments:

Reviewer: Aly, Hossam

The authors set out to investigate the evolution of inclined gas discs around eccentric binaries. In particular, they probe the regime where the initial (low mass) disc inclination is slightly below the critical inclination between the co-planar and polar alignment regimes. They first perform a number of SPH simulations to explore the full 3d behaviour of these systems, varying disc initial inclinations and binary eccentricities. They then use a 1d linear (in disc tilt) model to predict the long term evolution. The predictions from the linear model agree very well with the SPH results in terms of the maximum tilt as a function of binary eccentricity. They then use this model to construct a physical model for the binary system KH 15D, constraining the disc outer radius and viscosity coefficient. The results are sound and significant and I recommend the manuscript for publication. I do however have some minor comments that I would like the authors to address:

1-  3rd paragraph in the introduction: “The binary GG Tau may be misaligned by 25-30 from its circumbinary disc (Cazzoletti et al. 2017).”
GG Tau is a quadruple (possibly quintuple Di Folco et al. 2014) system. The authors perhaps mean the GG Tau A binary system. In which case the reference might need to be adjusted. Cazzoletti et al. 2017 examined a co-planar circumbinary disc, and their disagreement with the observed dust ring (Andrews et al. 2014) suggested that the system should be inclined. The 25-30 degrees inclination comes from Köhler 2011 astrometric fit (among other fits), and is indeed the best fit model in Aly et al. 2018 SPH simulations.

RESPONSE: We have changed from “binary GG Tau” to “binary GG Tau A” and have adjusted the references.

2- Section 3.2.3 “The upper-right hand panel” should just be the right hand panel. Same in section 3.2.4

RESPONSE: We have corrected this.

3- The authors ignore the dynamical effects on the binary which is reasonable because the disc mass is very low. However, run5 has an outer radius 8 times larger than the other simulations, which means the disc angular momentum is significantly larger in this case than the other runs. Do the authors still not see any dynamical effects on the binary in this run throughout the 2000 P_orb lifetime of the simulation? This would be interesting to note either way.

RESPONSE: Extending the disc outer radius by a factor of $8$ increases the disc angular momentum compared to the previous simulations. We investigated whether there are significant dynamical effects that the extended disc exerts on the binary. The maximum deviation from the initial binary inclination and eccentricity is $0.0072\degree$ and $0.0104$, respectively. Thus, there are no significant dynamical effects on the binary.

4- Figure 12 shows an excellent agreement between the maximum tilt obtained from the 1d linear model and the SPH simulations with low inclinations (for which the linear model is valid). However, as far as I can judge by eye, even the SPH simulations with higher inclinations (runs 2, 3, and 4) don’t seem to disagree too much. I think this would be interesting to point out.

RESPONSE: We have added a sentence at the end of the paragraph pointing out that there is some agreement with the linear model and the SPH simulations at higher initial tilt. 


5- Section 6 considers a physical model for the system KH 15D in which the inclination is just below critical and that it is not on the way to go polar. Is this just an assumption or is polar precession (libration) excluded by the observation? This is mentioned in the last sentence in the summary but I think it should be clarified in section 6 as well, not to keep the reader wondering.

RESPONSE:  If the disc tilt is above this critical value, then the disc will evolve to a polar (perpendicular) alignment with the binary. However, for this work, we only examine the conventional model where the disc or ring is precessing about a co-planar state

6- In Section 6.3, obtaining values of \alpha that are not very low depends on the strength of radial drift of the occulting dust particles. Perhaps it would be good to include the Stokes number explicitly in this case (it can be inferred from equ. 32 but I think the section would be benefit from explicitly stating the Stokes number). In particular with the chosen disc mass of 10^-3 and dust particles size of 50 micron one can estimate a value for St depending on r_out. If St ~ 1 to 0.1 then radial drift is expected to play a significant role, strengthening the conclusion of this section.

RESPONSE: The Stokes number for dust grains compares the stopping time to the dynamical time.  With our model parameters, we find that the stokes number is $6\times10^{-4}$. For these parameters, the dust is well coupled to the gas. The inward radial drift velocity due to gas drag is $10^{-6} \Omega r$.  The drift timescale is then of order $10^6$ years. Its numerical value in this case is not sensitive to $p$ for $0.5 \le p \le 1.5$. Shorter drift timescales occur for less massive discs. 
